KGUF: Simple Knowledge-aware Graph-based Recommender with User-based Semantic Features Filtering

The recent integration of Graph Neural Networks (GNNs) into recommendation has led to a novel family of Collaborative Filtering (CF) approaches, namely Graph Collaborative Filtering (GCF). Following the same GNNs wave, recommender systems exploiting Knowledge Graphs (KGs) have also been successfully empowered by the GCF rationale to combine the representational power of GNNs with the semantics conveyed by KGs, giving rise to Knowledge-aware Graph Collaborative Filtering (KGCF), which use KGs to mine hidden user intent. Nevertheless, empirical evidence suggests that computing and combining user-level intent might not always be necessary, as simpler approaches can yield comparable or superior results while keeping explicit semantic features. Under this perspective, user historical preferences become essential to refine the KG and retain the most discriminating features, thus leading to concise item representation. Driven by the assumptions above, we propose KGUF, a KGCF model that learns latent representations of semantic features in the KG to better define the item profile. By leveraging user profiles through decision trees, KGUF effectively retains only those features relevant to users. Results on three datasets justify KGUF's rationale, as our approach is able to reach performance comparable or superior to SOTA methods while maintaining a simpler formalization. Link to the repository: https://github.com/sisinflab/KGUF.

==> images/abl_depth.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}[inner frame sep=0pt]
    \begin{axis}[
    height=4.5cm,
    width=0.85*\linewidth,
    xlabel={max depth},
    ylabel={nDCG@10},
    ymin=0.22,
    ymax=0.27,
    ylabel near ticks,
    % yticklabel pos=right,  % <-- Added this line
    % xlabel near ticks
    symbolic x coords={1, 2, 5, 10, 15, 20, 100},
    xtick=data,
    scale only axis,
    legend cell align=left,
    /pgfplots/enlargelimits=false,
          legend style={legend pos=north west,font=\tiny}
    ]

    \addplot[name path=one_top,color=cambridgeblue,smooth,line width=1.5pt] table [col sep=tab,x index=1,y index=2] {images/csv/yahoo_depth_npr1_avg_max_min.tsv};
    \addplot[name path=one_down,color=brightube,smooth, line width=1.5pt] table [col sep=tab,x index=1,y index=3] {images/csv/yahoo_depth_npr1_avg_max_min.tsv};
    \addplot[name path=one_down,color=bananamania,smooth, line width=1.5pt] table [col sep=tab,x index=1,y index=4] {images/csv/yahoo_depth_npr1_avg_max_min.tsv};
    \legend{Average, Maximum, Minimum}
    \end{axis}    
    \pgfresetboundingbox
\path
  (current axis.south west) -- ++(-0.25in,-0.25in)
  rectangle (current axis.north east) -- ++(0.1in,0.1in);
\end{tikzpicture}
   \caption{Impact of max depth  on \textit{Yahoo! Movies}.}
    \label{fig:depth_abl}
\end{figure}





==> images/ablation_npr.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={NPR},
            ylabel={NDCG@10},
            ymin=0.235,
            ymax=0.265,
            ybar,
            bar width=10,
            grid=major,
            symbolic x coords={1, 2, 5, 10, 20}, % Specify the categories here
            xtick=data, % Show all categories on the X-axis
        ]

        \addplot table [col sep=tab, x index=0, y index=1] {images/csv/yahoo_npr_seed.tsv};

        \end{axis}
    \end{tikzpicture}
    \caption{Impact of $\eta$  on \textit{Yahoo! Movies}.}
    \label{fig:npr_ablation}
\end{figure}

==> images/bak_ablation_npr.tex <==
\begin{figure*}
\small
    \centering
    \begin{subfigure}{.4\linewidth}
        \centering
        \begin{tikzpicture}[inner frame sep=0pt]
    \begin{axis}[
    height=4.5cm,
    width=\linewidth,
    xlabel={NPR},
    ylabel={nDCG},
    ymin=0.235,
    ymax=0.265,
    ylabel near ticks,
    xlabel near ticks
    ]

    \addplot[color=red,smooth]  table [col sep=tab,x index=1,y index=3] {images/csv/yahoo_npr_aver_min_max.tsv};
    \addplot[name path=one_top,color=red!70,smooth] table [col sep=tab,x index=1,y index=4] {images/csv/yahoo_npr_aver_min_max.tsv};
    \addplot[name path=one_down,color=red!70,smooth] table [col sep=tab,x index=1,y index=2] {images/csv/yahoo_npr_aver_min_max.tsv};
    \addplot[red!50,fill opacity=0.5] fill between[of=one_top and one_down];    
    \end{axis}    
    \pgfresetboundingbox
\path
  (current axis.south west) -- ++(-0.25in,-0.25in)
  rectangle (current axis.north east) -- ++(0.1in,0.1in);
    \end{tikzpicture}
    \caption{}
    \label{fig:plausible-a}
    \end{subfigure}
    %\hfill
\caption{Impact of NPR  on \textit{Yahoo! Movies}.}
    \label{fig:alfabeta}
%\vspace{-0.75em}
\end{figure*}





==> tables/accuracy.tex <==
\begin{table*}
\small
    \caption{Comparison of accuracy perfomance between \framework and competing methods. All the differences betweeen \framework and the baselines are statistically significant based on paired t-tests ($p<0.05$) except for the values denoted with *.}
    \label{table:accuracy_full}
    \centerline{
\begin{tabular}{lllllllllllll}
\toprule
& \multicolumn{4}{c}{\textbf{Facebook Books}} & \multicolumn{4}{c}{\textbf{Yahoo! Movies}} & \multicolumn{4}{c}{\textbf{MovieLens 1M}} \\
\cmidrule(r){2-5} \cmidrule(lr){6-9} \cmidrule(l){10-13}
 & \textbf{nDCG} & \textbf{HR} & \textbf{Prec.} & \textbf{Recall} & \textbf{nDCG} & \textbf{HR} & \textbf{Prec.} & \textbf{Recall} & \textbf{nDCG} & \textbf{HR} & \textbf{Prec.} & \textbf{Recall} \\
%\midrule
\cmidrule(r){2-5} \cmidrule(lr){6-9} \cmidrule(l){10-13}
\textbf{Random} & 0.0074 & 0.0256 & 0.0027 & 0.0110 & 0.0065 & 0.0342 & 0.0036 & 0.0090 & 0.0096 & 0.0836 & 0.0091 & 0.0036 \\
\textbf{MostPop} & 0.0787 & 0.2535 & 0.0272 & 0.1117 & 0.1185 & 0.3238 & 0.0571 & 0.1501 & 0.1730 & 0.6537 & 0.1539 & 0.0773 \\
\textbf{BPR-MF} & 0.0945 & 0.2973 & 0.0333 & 0.1358 & 0.2303 & 0.5228 & 0.0965 & 0.2843 & 0.3100 & 0.8811 & 0.2686 & 0.1627 \\
\textbf{Item-kNN} & \underline{0.1039} & \underline{0.3353} & \underline{0.0378} & \underline{0.1556} & 0.2258 & 0.5033 & 0.0929 & 0.2658 & 0.2932 & 0.8504 & 0.2564 & 0.1490 \\
\textbf{KGFlex} & 0.0712 & 0.2235 & 0.0246 & 0.1001 & 0.1758 & 0.4360 & 0.0680 & 0.2022 & 0.0111 & 0.1058 & 0.0122 & 0.0053 \\
\textbf{kaHFM} & 0.0843 & 0.2776 & 0.0300 & 0.1221 & 0.2085 & 0.5064 & 0.0902 & 0.2621 & 0.2992 & 0.8654 & 0.2581 & 0.1526 \\
\textbf{LightGCN} & 0.0969 & 0.3170 & 0.0355 & 0.1435 & 0.2230 & 0.5085 & 0.0937 & 0.2712 & 0.3081 & 0.8813 & 0.2683 & 0.1614 \\
\textbf{DGCF} & 0.1001 & 0.3192 & 0.0354 & 0.1444 & 0.2356 & 0.5308 & 0.0981 & 0.2848 & \underline{0.3124} & 0.8819 & \underline{0.2714} & 0.1637 \\
\textbf{KGIN} & 0.1023 & 0.3112 & 0.0356 & 0.1448 & \underline{0.2368} & \underline{0.5500}$^*$ & \underline{0.1006}$^*$ & \textbf{0.2971} & 0.3082 & \underline{0.8854} & 0.2695 & \underline{0.1638} \\
\textbf{KGTORe} & \textbf{0.1188} & \textbf{0.3601} & \textbf{0.0414} & \textbf{0.1698} & \textbf{0.2471} & \textbf{0.5566} & \textbf{0.1018} & \underline{0.2944} & 0\textbf{.3212} & \textbf{0.8957} & \textbf{0.2772} & \textbf{0.1710} \\
\textbf{\framework} & \textbf{0.1183} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.2564} & \textbf{0.0} & \textbf{0.0} & \underline{0.0} & \textbf{.3286} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\
\bottomrule
\end{tabular}
}
\end{table*}
